Proto-exact and parabelian categories

Proto-exact and parabelian categories serve as non-additive analogues of exact and quasi-abelian categories, respectively. They give rise to algebraic K-theory and Hall algebras similarly to the additive setting. We show that every parabelian category admits a canonical proto-exact structure and we study several classes of parabelian categories, including categories of normed and Euclidean vector spaces, pointed closure spaces and pointed matroids, Hermitian vector bundles over rings of integers. We also examine finitary algebraic categories arising in Arakelov geometry and provide a criterion for determining when such a category is parabelian. In particular, we prove that the categories of pointed convex spaces and absolutely convex spaces are parabelian.

==> commands.tex <==
\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{etoolbox,bbm,xspace,scalerel}
\RequirePackage{version,xparse}
%\RequirePackage[a4paper,margin=1.35in]{geometry}
\makeatletter

%%%% Theorem environments
\ifx\theorem\undefined
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}{Conjecture}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{question}[theorem]{Question}
\theoremstyle{remark}
\newtheorem{rmr}[theorem]{Remark}
\fi


%%%% Auxiliary commands
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}} %define math command
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}
\def\opn{\operatorname}
\def\opr#1#2{\dmat#1{\opn{#2}}}
\def\DMO{\opr}
\def\csopr#1#2{\csdmat{#1}{\opn{#2}}}
\def\oper#1{\csopr{#1}{#1}}
\def\operl{\forcsvlist\oper}
\def\redef#1{\csletcs{t@#1}{#1}\csdmat{#1}{\csuse{t@#1}}}
\newcommand\envalias[2]{\newenvironment{#1}{\begin{#2}}{\end{#2}}}


%%%% Operators. Usage: \GL
\forcsvlist\oper{
Vect,Mod,Rep,Ab,Grp,Com,Set,Top,Sch,Coh,Qcoh,Ob,Ring,Alg,
Map,Hom,End,Aut,Ext,Cat,Sh,Ind,RHom,Fun,Var,rad,
Ker,Im,Re,deg,Tr,det,rk,diag,im,coker,tr,cone,add,
sk,cosk,colim,Res,Gal,Coker,dlog,sgn,Li,
GL,SL,PGL,Gr,Lib,Conv,Sol,Tor,
Max,Spec,Proj,Ass,Ann,Quot,Pic,Sym,MHS,MHM,
td,Td,ch,Supp,supp,vol,trdeg,lc,NS,Loc,Iso,per,gr,Der,Lie,
Log,Exp,Pow,ord,lcm,VB,Hilb,cl,SU,SO,Ad,ad,id,Span,Arg,Bl,wt,Cone,
coim,Coim,eq,coeq,Eq,Coeq}

\opr\Id{id}
\opr\lHom{\lb{Hom}}
\opr\lEnd{\lb{End}}
\opr\lAut{\lb{Aut}}
\opr\lIso{\lb{Isom}}
\opr\hgt{ht}
\opr\chr{char}
\opr\udim{\mathbf{dim}}
\opr\cls{\mathsf{cl}}
\opr\mmod{mod}
\opr\Et{\mathsf{Et}}
\def\sign{\sgn}
\opr\spn{span}

\dmat\Gm{\mathbb G_{\mathrm m}}
\dmat\pt{\mathbf{pt}}
\def\opfrak#1{\csdef{#1}{\mathfrak{#1}}}
\forcsvlist\opfrak{gl,sl,su,so}
\def\oprm#1{\csdef{#1}{\mathrm{#1}}}
\forcsvlist\oprm{op,nil,et,sep,ab,top,tf,}
\def\st{\mathrm{s}}
\def\sst{\mathrm{ss}}
\def\Ta{T^{\mathrm a}} %tensor algebra
\def\Tc{T^{\mathrm c}} %tensor coalgebra
\def\Vecf{\Vect_{\mathrm f}}

%%%% Arrows
\def\mto{\mapsto}
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\emb{\hookrightarrow}
\def\lemb{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\def\isoto{\xto{\,\smash{
	\raisebox{-3pt}{\ensuremath{\scriptstyle\sim}}
}\,}}
\RequirePackage{mathtools}
\def\xmto{\xmapsto}
\def\xlto{\xleftarrow}
\def\xemb{\xhookrightarrow}
\def\xonto#1{\xto{#1}\mathrel{\mkern-14mu}\to}
\def\dashto{\dashrightarrow}
\def\dto{\dashrightarrow}
\def\dashlto{\dashlefttarrow}
\def\dlto{\dashlefttarrow}

%%% Symbols
\dmat\es{\varnothing}%{\emptyset}
\def\bs{\backslash}
\def\ms{\backslash}
\def\sbs{\subset}
\def\sps{\supset}
\def\sbe{\subseteq}
\def\spe{\supseteq}
\redef{iff}
\dmat\imp{\implies}
\dmat\xx{\times}
\dmat\dd{\partial}
\def\pd#1{\frac\dd{\dd#1}}
\def\iso{\simeq}
\def\isoc{\cong} %canonical isomorphism
\def\bop{\bigoplus}
\def\ilim{\varprojlim} %inverse limit
\def\dlim{\varinjlim} %direct limit
\def\ts{\otimes}
\def\bts{\bigotimes}
\def\lb{\underline}
\def\ub{\overline}
\def\ubar#1{\mkern1.5mu\overline%
	{\mkern-1.5mu#1\mkern-1.5mu}\mkern1.5mu}
\def\oh{{\frac12}}
\def\toh{{\tfrac12}}
\dmat\one{\mathbbm1}
\def\qt{\delimiter"502F30E\mathopen{}} %/correct spacing
\def\partof{\vdash}
\def\adj{\mathrel{\tikz
\draw[line cap=round](0,0)--(0,1.5ex)(0,.75ex)--(-1.5ex,.75ex);}}
%\def\adj{\mathrel{\relbar\mkern-14mu\vcenter{\hbox{$\dashv$}}}}
\def\what{\widehat}
\def\tl{\tilde}
\def\wtl{\widetilde}
\def\inv{^{-1}}
\def\trp{^{\mathsf T}} %transpose
\dmat\bul{\bullet}
\def\GIT{/\!\!/}
\def\git{\GIT}
\def\qbinom{\genfrac{[}{]}{0pt}{}}
\def\ac{{\tiny\raisebox{2pt}{\textup{!`}}}}%anti-shriek
\def\m{\wedge}
\def\j{\vee}
\def\blank{\scalebox{.8}{$-$}} %blank argument

\def\upc{\tikz{\draw[->,>=latex'](0,0)--(0,.3)}}
%requires \usetikzlibrary{arrows}
\def\upc#1{\left\uparrow#1\right.}%upper closure
\def\loc#1{\left\downarrow#1\right.}%lower closure
\def\cupp{\!\smallsmile\!} %cup product
\def\capp{\!\smallfrown\!} %cap product

\NewDocumentCommand\cscale{O{.7}O{0pt}m}
%Central scale: #1-scale, #2-raise, #3-argument
{\mathbin{\ThisStyle{\vcenter{\hbox{%
  \raisebox{#2}{\scalebox{#1}{$\SavedStyle#3$}}%
}}}}}

\def\sbul{\cscale[.7][1pt]{\bullet}}
\def\dual{^{\scalerel*\vee*}}
%\def\dual{^{\cscale[.8]{\vee}}}



\usepackage[T2A]{fontenc} %T2A, OT2
\def\sha{\mathbin{\textup\cyrsh}}

\let\t@sum\sum
\def\sum{\@ifstar{\t@sum\nolimits}\t@sum}

\newcommand\tcd[2][]{%
  \begin{tikzcd}[#1,ampersand replacement=\&]#2\end{tikzcd}}

\newenvironment{ctikzcd}
	{\center\tikzcd}{\endtikzcd\endcenter}

\newcommand\edge[2][1.5em]{%\xrightarrow without tip
  \tcd[cramped,column sep=#1]{\rar[-,"#2"]\&{}}}

%%%% Aphabets: \bA,\cA,\fA,\bfA,\sA
\def\flist#1#2{\expandafter\forcsvlist\expandafter#1\expandafter{#2}}
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\def\deffrak#1{\csdmat{f#1}{\mathfrak{#1}}}
\def\defbf#1{\csdmat{bf#1}{\mathbf{#1}}}
\def\defsf#1{\csdmat{s#1}{\mathsf{#1}}}
\def\defrm#1{\csdmat{r#1}{\mathrm{#1}}}
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}\defbf{#1}%
  \defsf{#1}\defrm{#1}}

\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

\def\deflbf#1{\csdmat{b#1}{\mathbf{#1}}} %lower case bf
\forcsvlist\deflbf{a,b,c,d,e,g,h,i,j,k,l,n,o,p,q,r,s,t,u,v,w,x,y,z}
\forcsvlist\defbf{f,k,m} %\bff,\bfk,\bfm
%\dmat\bk{\mathbbm k}
\dmat\bk{\Bbbk}
\defrm{i} %\ri

%%%% Greek letters
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\la\lambda
\dmat\ta\tau
\dmat\hi\chi
\dmat\eps\varepsilon
\dmat\ep\epsilon
\dmat\io{\iota}
\dmat\vi\phi
\dmat\te\theta
\dmat\ksi\xi
\dmat\si\sigma
\dmat\om\omega
\dmat\Ga\Gamma
\dmat\La\Lambda
\dmat\De\Delta
\dmat\Om\Omega
\dmat\Si{\Sigma}
\dmat\ze\zeta
\dmat\Te{\Theta}
\dmat\Na{\nabla}
\dmat\kp{\kappa}
\forcsvlist\redef{Phi,Psi,pi,mu,nu,rho}

%%%% Structures
\RequirePackage{mleftright} %better spaces
\def\lr#1#2#3{\mleft#1#2\mright#3}
\def\set#1{\lr\{{#1}\}}
%\def\sets#1#2{\set{#1\,\lr|{\,\vphantom{#1}#2}.}}
\def\sets#1#2{\set{#1\,\middle|\,#2}}
\def\ang#1{\lr\langle{#1}\rangle}
\def\angs#1#2{\ang{#1\col#2}}
\def\rbr#1{\lr({#1})} %round bracket
\def\sbr#1{\lr[{#1}]} %square bracket
\def\brc{\set} %curly bracket, braces
\def\cbr{\set}
\def\emp{\cdot,\cdot} %empty parameters
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\n#1{\left\lvert#1\right\rvert}
\def\nn#1{\left\lVert#1\right\rVert}

\def\rbig#1{\big(#1\big)}
\def\rBig#1{\Big(#1\Big)}
\def\rbigg#1{\bigg(#1\bigg)}
\def\sth#1#2{\lr.{#1}|_{#2}}

\def\nspc#1{\hspace{-2.5pt}#1\hspace{-2.5pt}}%neg. space
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{(\nspc{(#1)})} %formal Laurent series ((#1))
\def\cps#1{\{#1\}} %convergent power series
\def\cls#1{(\nspc{\cps{#1}})} %convergent Laurent series
\def\angg#1{\ang{\nspc{\ang{#1}}}}
\def\nop#1{\left.\col\nspc{#1}\col\right.}%normal oper product
\def\nop#1{\left.\col\mathrel{#1}\col\right.}
%\def\nop#1{\col\mathrel{#1}\col}


\def\matr#1{\begin{matrix}#1\end{matrix}}
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bmat#1{\begin{bmatrix}#1\end{bmatrix}}
\def\vmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\smatr#1{\begin{smallmatrix}#1\end{smallmatrix}}
\def\smat#1{\rbr{\smatr{#1}}}
\def\pmatv#1#2{\left(\matr{#1}
	\hspace{.5ex}\middle|\hspace{.3ex}
	\matr{#2}\right)}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2
%\def\eq#1{\begin{equation}#1\end{equation}} %used for equalizers


%%%% Diff
\def\br{\ \vspace{-.5ex}} %break after itemize
\def\dir#1#2{\noindent\textbf{(#1)$\implies$(#2).}}
\def\clm#1{\noindent\textbf{(#1)}\xspace} %claim, \cl should be used for classes
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\qq#1{\lqq#1\rqq}
\def\tpdf{\texorpdfstring} %hyperref
\def\hl{\noindent\rule{\textwidth}{1pt}}

%%%% Words and phrases
%\def\ie{i.e.\@\xspace} %id est
%\def\eg{e.g.\@\xspace} %exempli gratia
%\def\cf{cf.\@\xspace} %confer
\def\ie{i.e.,\,} %id est
\def\eg{e.g.\ } %exempli gratia
\def\cf{cf.\ } %confer
\def\lci{l.c.i.\@\xspace}
%\def\fd{f.d.\@\xspace} % used for \mathfrak{d}
\def\etale{\'etale\xspace}
\def\qis{quism\xspace} %quasi-isomorphism
\def\wrt{with respect to\xspace}
\def\hint{\noindent\textbf{Hint:}\xspace}
\def\Wlog{Without loss of generality\xspace}
\def\tfae{the following are equivalent\xspace}
\def\nbd{neighborhood\xspace}

%%%% Citations
\def\defcite#1#2{%\defcite\moz{mozgovoy_DT}
	\DeclareDocumentCommand{#1}{o}
		{\IfValueTF{##1}{\cite[##1]{#2}}{\cite{#2}}\xspace}
}
\def\eprint#1{\href{https://arxiv.org/abs/#1}{\ttfamily#1}}

%%%% Colons
\mathchardef\col=\mathcode`:
\def\colon{\nobreak \mskip 2mu\mathpunct {}\nonscript \mkern -\thinmuskip {\col}\mskip 6muplus1mu\relax}

\RequirePackage{mathtools} %for \coloneqq
\def\ordinarycolon{\col} %used in \coloneqq and \vcentcolon

{\catcode`:=\active\makeatletter
    \gdef:{\@ifnextchar={\coloneqq\@gobble}{\colon}}}
\AtBeginDocument{\mathcode`:="8000}

\mathchardef\latexequal=\mathcode`=
{\catcode`==\active\makeatletter
    \gdef={\@ifnextchar:{\eqqcolon\@gobble}{\latexequal}}}
\AtBeginDocument{\mathcode`=="8000}


%%%% Indexed definition \idef{name}{optional name}
\DeclareDocumentCommand{\idef}{mo}{%
	\ifmmode#1\else\textit{#1}\fi%
	\IfValueTF{#2}{\index{#2}}{\index{#1}}%
}


%%% Notes
\ifx\note\undefined
\RequirePackage[framemethod=TikZ]{mdframed}
\mdfsetup{backgroundcolor=brown!10, linewidth=0, skipabove=1ex, roundcorner=5pt}

\theoremstyle{definition}
\newmdtheoremenv[innertopmargin=-2pt]{note}{Note}
\newenvironment{notes}{\begin{note}}{\end{note}}

\newenvironment{comm}[1][brown!10]
    {\begin{mdframed}[backgroundcolor=#1,innertopmargin=5pt]}
    {\end{mdframed}}
\long\def\memo#1{\comm#1\endcomm}
\def\red#1{\textcolor{red}{#1}}
\fi

%custom number side in equations, manual number: \tag{name}
\makeatletter
\def\leqnomode{\tagsleft@true\let\veqno\@@leqno}
\def\reqnomode{\tagsleft@false\let\veqno\@@eqno}
\makeatother


%custom theorem, can be used to list axioms (with labels)
\ifx\customthm\undefined
\theoremstyle{plain}
\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\def\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\fi

% subsection command
\DeclareDocumentCommand\sec{o}{
  \IfValueTF{#1}
    {\subsection{#1}}
    {\subsection{}\hspace{-1ex}}}

% short names for theorems
\def\shortThm{
\envalias{thm}{theorem}
\envalias{thr}{theorem}
\envalias{dfn}{definition}
\envalias{lmm}{lemma}
\envalias{crl}{corollary}
\envalias{prp}{proposition}
}

\makeatother

%%%% Tikz %%%%
%\long\def\command#1{\providecommand{#1}{}\renewcommand{#1}}
\newcommand\vcenterx[1]{\ensuremath{\vcenter{\hbox{#1}}}}
\newcommand\btikz[2][]{\vcenterx{\tikz[#1]{#2}}} %base line
\newcommand\ctikz[2][]{\begin{center}\tikz[#1]{#2}\end{center}}


